Optimal and Private Learning from Human Response Data

Item response theory (IRT) is the study of how people make probabilistic decisions, with diverse applications in education testing, recommendation systems, among others. The Rasch model of binary response data, one of the most fundamental models in IRT, remains an active area of research with important practical significance. Recently, Nguyen and Zhang (2022) proposed a new spectral estimation algorithm that is efficient and accurate. In this work, we extend their results in two important ways. Firstly, we obtain a refined entrywise error bound for the spectral algorithm, complementing the `average error' $\ell_2$ bound in their work. Notably, under mild sampling conditions, the spectral algorithm achieves the minimax optimal error bound (modulo a log factor). Building on the refined analysis, we also show that the spectral algorithm enjoys optimal sample complexity for top-$K$ recovery (e.g., identifying the best $K$ items from approval/disapproval response data), explaining the empirical findings in the previous work. Our second contribution addresses an important but understudied topic in IRT: privacy. Despite the human-centric applications of IRT, there has not been any proposed privacy-preserving mechanism in the literature. We develop a private extension of the spectral algorithm, leveraging its unique Markov chain formulation and the discrete Gaussian mechanism (Canonne et al., 2020). Experiments show that our approach is significantly more accurate than the baselines in the low-to-moderate privacy regime.

==> extra.tex <==



==> pics/subsample_graph.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[scale=0.75,x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,234); %set diagram left start at 0, and has height of 234

%Straight Lines [id:da8690730661234298] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=3]    (224.08,113.49) -- (285.39,207.57) ;
%Straight Lines [id:da07245996699159574] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=3]    (265.24,18.94) -- (401.99,167.46) ;
%Straight Lines [id:da9139262610121521] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (392.99,18.94) -- (288.82,211.39) ;
%Straight Lines [id:da80922284178616] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=3]    (430.72,76.24) -- (288.82,211.39) ;
%Straight Lines [id:da521914845664337] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (430.72,76.24) -- (265.67,13.68) ;
%Straight Lines [id:da03721851621608918] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (401.99,167.46) -- (224.08,113.49) ;
%Straight Lines [id:da5925909409695378] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (224.08,113.49) -- (392.99,18.94) ;
%Straight Lines [id:da30816922375981703] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (265.67,13.68) -- (288.82,211.39) ;
%Straight Lines [id:da4912390283163601] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (430.72,76.24) -- (401.99,167.46) ;
%Straight Lines [id:da7234813617905078] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0 ]   (430.72,76.24) -- (392.99,18.94) ;
%Straight Lines [id:da9062773198646448] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (224.51,104.42) -- (265.24,18.94) ;
%Straight Lines [id:da5816945758963241] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=3]    (265.67,13.68) -- (392.99,18.94) ;
%Straight Lines [id:da19713143195110017] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.13 ]   (288.82,211.39) -- (401.99,167.46) ;
%Straight Lines [id:da8221937962330423] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.25 ][line width=0.75]    (392.99,18.94) -- (401.99,167.46) ;
%Straight Lines [id:da4424950560993848] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=2.25]    (224.08,113.49) -- (430.72,76.24) ;
%Straight Lines [id:da9850720609864463] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=3]    (433,73.67) -- (392.99,18.94) ;
%Flowchart: Connector [id:dp7618772421632545] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (217.01,111.75) .. controls (217.01,107.7) and (220.37,104.42) .. (224.51,104.42) .. controls (228.66,104.42) and (232.01,107.7) .. (232.01,111.75) .. controls (232.01,115.8) and (228.66,119.09) .. (224.51,119.09) .. controls (220.37,119.09) and (217.01,115.8) .. (217.01,111.75) -- cycle ;
%Flowchart: Connector [id:dp5538521128138689] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (257.74,18.94) .. controls (257.74,14.89) and (261.1,11.6) .. (265.24,11.6) .. controls (269.38,11.6) and (272.74,14.89) .. (272.74,18.94) .. controls (272.74,22.99) and (269.38,26.27) .. (265.24,26.27) .. controls (261.1,26.27) and (257.74,22.99) .. (257.74,18.94) -- cycle ;
%Flowchart: Connector [id:dp24937791431813472] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (385.49,18.94) .. controls (385.49,14.89) and (388.85,11.6) .. (392.99,11.6) .. controls (397.13,11.6) and (400.49,14.89) .. (400.49,18.94) .. controls (400.49,22.99) and (397.13,26.27) .. (392.99,26.27) .. controls (388.85,26.27) and (385.49,22.99) .. (385.49,18.94) -- cycle ;
%Flowchart: Connector [id:dp1635771887609836] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (425.5,73.67) .. controls (425.5,69.62) and (428.86,66.33) .. (433,66.33) .. controls (437.14,66.33) and (440.5,69.62) .. (440.5,73.67) .. controls (440.5,77.72) and (437.14,81) .. (433,81) .. controls (428.86,81) and (425.5,77.72) .. (425.5,73.67) -- cycle ;
%Flowchart: Connector [id:dp10130223253846182] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (394.49,167.46) .. controls (394.49,163.41) and (397.85,160.12) .. (401.99,160.12) .. controls (406.14,160.12) and (409.49,163.41) .. (409.49,167.46) .. controls (409.49,171.51) and (406.14,174.79) .. (401.99,174.79) .. controls (397.85,174.79) and (394.49,171.51) .. (394.49,167.46) -- cycle ;
%Flowchart: Connector [id:dp14155906642820693] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (277.89,207.57) .. controls (277.89,203.52) and (281.25,200.24) .. (285.39,200.24) .. controls (289.53,200.24) and (292.89,203.52) .. (292.89,207.57) .. controls (292.89,211.62) and (289.53,214.91) .. (285.39,214.91) .. controls (281.25,214.91) and (277.89,211.62) .. (277.89,207.57) -- cycle ;




\end{tikzpicture}

